Robust Training under Label Noise by Over-parameterization

Recently, over-parameterized deep networks, with increasingly more network parameters than training samples, have dominated the performances of modern machine learning. However, when the training data is corrupted, it has been well-known that over-parameterized networks tend to overfit and do not generalize. In this work, we propose a principled approach for robust training of over-parameterized deep networks in classification tasks where a proportion of training labels are corrupted. The main idea is yet very simple: label noise is sparse and incoherent with the network learned from clean data, so we model the noise and learn to separate it from the data. Specifically, we model the label noise via another sparse over-parameterization term, and exploit implicit algorithmic regularizations to recover and separate the underlying corruptions. Remarkably, when trained using such a simple method in practice, we demonstrate state-of-the-art test accuracy against label noise on a variety of real datasets. Furthermore, our experimental results are corroborated by theory on simplified linear models, showing that exact separation between sparse noise and low-rank data can be achieved under incoherent conditions. The work opens many interesting directions for improving over-parameterized models by using sparse over-parameterization and implicit regularization.

==> notations.tex <==
\newcommand{\myparagraph}[1]{\noindent\textbf{#1.}}

% \graphicspath{ {./figs/} }

% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

\def\0{\textbf{0}}
\def\1{\textbf{1}}
%\def\11{\mathbb{1}}
\def\a{\boldsymbol{a}}
%\def\b{\boldsymbol{b}}
\def\c{\boldsymbol{c}}
\def\e{\boldsymbol{e}}
\def\f{\boldsymbol{f}}
\def\v{\boldsymbol{v}}
\def\p{\boldsymbol{p}}
\def\q{\boldsymbol{q}}
\def\s{\boldsymbol{s}}
\def\t{\boldsymbol{t}}
\def\u{\boldsymbol{u}}
\def\v{\boldsymbol{v}}
\def\w{\boldsymbol{w}}
\def\x{\boldsymbol{x}}
\def\y{\boldsymbol{y}}
\def\z{\boldsymbol{z}}

\def\A{\boldsymbol{A}}

\def\cA{\mathcal{A}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cH{\mathcal{H}}
\def\cT{\mathcal{T}}
\def\cS{\mathcal{S}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}

\def\st{\textrm{s.t.}}

\newcommand{\RR}{I\!\!R} %real numbers
\newcommand{\Nat}{I\!\!N} %natural numbers
\newcommand{\CC}{I\!\!\!\!C} %complex numbers

%\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}

\renewcommand{\mathbf}{\boldsymbol}

\newcommand{\conv}{\circledast}
\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }


\newcommand{\reals}{{\mathbb R}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\E}{\mathbb{E}}

%\newcommand{\eps}{\varepsilon}
\renewcommand{\Re}{{\mathbb R}}
\newcommand{\Cp}{\bb C}
\newcommand{\Z}{\bb Z}
\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1_{#1}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{\col}{\mathrm{col}}
% to declare new operator
% \DeclareMathOperator{\xxx}{xxx}

%% Other definitions

\newcommand{\event}{\mc E}

\newcommand{\im}{\mathrm{i}}
\newcommand{\rconcave}{r_\fgecap}
\newcommand{\Lconcave}{\mc L^\fgecap}
\newcommand{\rconvex}{r_\fgecup}
\newcommand{\Rconvex}{R_\fgecup}
\newcommand{\Lconvex}{\mc L^\fgecup}

\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\ol}{\overline}


\newcommand{\betaconcave}{\beta_\fgecap}
\newcommand{\betagrad}{\beta_{\mathrm{grad}}}

\newcommand{\norm}[2]{\left\| #1 \right\|_{#2}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\innerprod}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\prob}[1]{\bb P\left[ #1 \right]}
\newcommand{\expect}[1]{\bb E\left[ #1 \right]}
\newcommand{\function}[2]{#1 \left(#2\right}
\newcommand{\integral}[4]{\int_{#1}^{#2}\; #3\; #4}

\newcommand{\mr}{\mathrm}
\newcommand{\inprod}[2]{\langle#1,#2\rangle}
\newcommand{\parans}[1]{\left(#1\right}


\newtheorem{remark}{Remark}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}

==> sections/methods.tex <==

\section{Main Ideas \& Contributions}
\label{sec:contribution}


%Despite the great benefits, over-parameterization brings critical issues when learning from data that is corrupted.Consider the task of image classification where some of the images in the training set are mislabeled (e.g., some images of cats are labeled as dogs). 


\paragraph{Problem setup.} Given a training dataset $\{(\x_i, \y_i)\}_{i=1}^N$, with $\x_i$ being an input and $\y_i$ being the corresponding (possibly corrupted) one-hot label, a standard approach in deep learning is to train a deep neural network $f(\cdot; \,\mb \theta)$ via solving an optimization problem with respect to (w.r.t.) the network parameter $\mb \theta$ as follows:
 \setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
 \setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}
\begin{equation}\label{eq:model}
    \min_{\mb \theta}\; L(\mb \theta) \;=\; \frac{1}{N} \sum_{i=1}^N \ell\Big(f(\x_i; \, \mb \theta), \;\y_i\Big),
\end{equation}
where $\ell(\cdot, \cdot)$ is a loss function that measures the distance between network output $f(\x_i; \, \mb \theta)$ and the label $\y_i$. For classification, we typically use the cross-entropy loss, denoted by $\ell_{\mathrm{CE}}(\cdot, \cdot)$, while sometime we use the mean-squared error (MSE) loss, denoted by $\ell_{\mathrm{MSE}}(\cdot, \cdot)$. As we observe, the overparameterization of $\mb \theta \in \bb R^d$ with $d \gg N$, means that there are infinite solutions of \eqref{eq:model}. As such, the high expressive power of over-parameterized models implies that the network tends to overfit the labels especially when $\y_i$ is corrupted, with $f(\x_i; \mb \theta) \approx \y_i$ for all $i=1,\cdots,N$. Therefore, overfitting to corruption inevitably leads to a poor generalization performance \cite{zhang2021understanding}. 

In contrast, if the label $\mb y_i$ is corrupted, we desire the learned network $f(\x_i; \, \mb \theta_\star)$ is able to correct the wrong labels rather than overfitting, in the sense that
\begin{align*}
    \underset{\textbf{corrupted label}}{\mb y_i} \;=\; \underset{ \textbf{correct output} }{f(\x_i; \, \mb \theta_\star)} \;+\; \underset{ \textbf{sparse label noise} }{\mb s_{\star i}}.
\end{align*}
Here, we suppose $f(\x_i; \, \mb \theta_\star)$ is an oracle network that can always predict the correct labels from any input $\mb x_i$, and the noise $\mb s_i$ is \emph{sparse} because the difference between two one-hot vectors $\mb y_i$ and $f(\x_i; \, \mb \theta_\star)$ would be two sparse.

%both $\mb y_i$ and $f(\x_i; \, \mb \theta_\star)$ are one-hot vectors so that their difference is still expected to be (i.e., two) sparse.


\paragraph{The main idea of our approach.} To deal with corruption in the overparameterized regime, our idea is simply to use an extra variable $\mb s_i$ to model the label noise $\mb s_{\star i}$ and enforce sparsity on $\mb s_i$ for optimization, so that we can correct the label noise and prevent the overparameterized network $f(\mb x;\mb \theta)$ from overfitting the wrong labels. While there are many ways to enforce sparsity on $\mb s_i$ such as using $\ell_1$-norm penalty, recent work \cite{you2020robust} suggests that a naive $\ell_1$-regularization approach degrades the performance and \emph{cannot} prevent overfitting. Instead of explicitly enforcing sparsity on the noise, inspired by a line of recent work \cite{vaskevicius2019implicit,zhao2019implicit,you2020robust}, our approach is to overparameterize $\mb s_i = \u_i \odot \u_i - \v_i \odot \v_i $ to \emph{implicitly} encourage sparsity on $\mb s_i$, and optimize the following training loss
\begin{equation}\label{eq:main_model} 
    \min_{\mb \theta, \{\u_i, \v_i\}_{i=1}^N} L(\mb \theta, \{\u_i, \v_i\}_{k=1}^N)
\end{equation}
with $\odot$ denoting an entry-wise Hadamard product and 
\begin{align*}
\small
    L(\mb \theta, \{\u_i, \v_i\}) =\frac{1}{N} \sum_{i=1}^N \ell (f(\x_i;\mb \theta)  + \u_i \odot \u_i - \v_i \odot \v_i,\y_i ).
\end{align*}
We term our method ``Sparse Over-Parameterization'' (SOP).
%The idea is simple: the observed label $\y_i$ is decomposed as the summation of two terms, where the first term $f(\x_i; \,\mb \theta)$ aims to produce the clean label, and the second term $\u_i \odot \u_i - \v_i \odot \v_i$ aims to produce label corruption (i.e., difference between clean and corrupted labels).The term $\u_i \odot \u_i - \v_i \odot \v_i$ can be interpreted as an over-parameterization of label corruption for the purpose of modeling sparsity. 


%Specifically, the terms $\u_i \odot \u_i$ and  $- \v_i \odot \v_i$ capture the positive and negative entries of the corruption, respectively, and the product form of $\u_i \odot \u_i$ (resp., $\v_i \odot \v_i$) enables it to easily compose corruption entries with a small value of $\u_i$ (resp., $\v_i$). 


%where $\ell(\cdot, \cdot)$ is the cross-entropy loss and  
%Ideally, the model should only fit to clean labels and should \emph{not} overfit, i.e., $f(\x_i; \mb \theta) \ne \y_i$, if $\y_i$ is corrupted. 
%However, because of the high expressive power of over-parameterized models, the solution to \eqref{eq:model} will ``memorize'' all corrupted labels, i.e., with $f(\x_i; \mb \theta) \approx \y_i$ for all $i \in \{1, \ldots, N\}$ \cite{zhang2021understanding}.
%Overfitting to corruption inevitably leads to a poor generalization performance. 

% \paragraph{This work: Robustness via over-parameterization. }
% \paragraph{Robustness by over-parameterization. }
%This paper presents a method to extend the power of sparse modeling for robustness to over-parameterized models.
%Instead of modeling sparsity with a loss function, our approach is to introduce a label corruption term with a particular over-parameterized form to encourage sparsity.
%For the image classification model \eqref{eq:model}, our approach is to solve the optimization problem
%\begin{equation}\label{eq:main_model}
%    \min_{\mb \theta, \{\u_i, \v_i\}_{i=1}^N} \frac{1}{N} \sum_{i=1}^N \ell\Big(f(\x_i; \,\mb \theta)  + \u_i \odot \u_i - \v_i \odot \v_i, \,\y_i\Big),
%\end{equation}
%where $\ell(\cdot, \cdot)$ can be commonly used cross-entropy or mean-squared-error losses and $\odot$ represents entry-wise multiplication of the vectors. 


% \paragraph{Role of algorithmic bias.}
At the first glance, our SOP approach is seemingly problematic, because adding more learnable parameters $\{\u_i, \v_i\}_{i=1}^N$ to an overparameterized network $f(\cdot, \mb \theta)$ would exaggerate rather than alleviate the overfitting issue. Against our conventional wisdom that more overparametrization leads to more overfitting, it is surprisingly that our (stochastic) gradient descent (GD) learning algorithm has \emph{implicit bias} towards regularized minimum $\ell_2$-norm solutions for $\mb u_{i}$ and $\mb v_{i}$ \cite{xx}. Thus, with $\norm{\mb s_{\star i}}{1} = \norm{ \mb u_{\star i} }{2}^2 + \norm{\mb v_{\star i} }{2}^2 $, it leads to the minimum $\ell_1$-norm solution of $\mb s_{\star i}$, so that our solution $\mb s_{\star i}$ is sparse and recovers the sparse label noise.
%Moreover, the nonnegativity of $\mb u_{\star i} \odot \mb u_{\star i}$ and $\mb v_{\star i} \odot \mb v_{\star i}$ suggests that they can capture the wrong and correct label entries, respectively. 
Technically, we run gradient descent on the proposed objective starting from small initializations for $\mb \theta, \{\u_i, \v_i\}_{i=1}^N$, with
\begin{equation}\label{eq:main_algorithm}
\begin{split}
    \mb \theta &\leftarrow \mb \theta - \eta \cdot \frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \mb \theta},\\
    \u_i &\leftarrow \u_i - \alpha \eta \cdot \frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \u_i},~~i=1, \ldots, N,\\
    \v_i &\leftarrow \v_i - \alpha \eta \cdot\frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \v_i},~~i=1, \ldots, N.\\
\end{split}
\end{equation}
By using \emph{discrepant} learning rates (i.e., the tuning parameter $\alpha>0,\;\alpha \not = 1$) for each learning parameter, we demonstrate that the GD method imposes \emph{implicit regularization} on $\mb \theta, \{\u_i, \v_i\}_{i=1}^N$.  As such, the implicit regularization will prevent overfitting and our gradient descent will converge to optimal solutions with the desired properties \cite{xx}. In \Cref{sec:experiments}, the effectiveness of our approach for dealing with label noise in image classification will be demonstrated on a variety of datasets, matching the state-of-the-art performance with very few hacks.

%in \Cref{sec:experiments}, for image classification we demonstrate that the stochastic variant of the gradient descent can also effectively recover the underlying sparse corruptions on a variety of datasets with both synthesized and real noisy labels.


% Moreover, one benefit of such a Hadamard product over an $\ell_1$ penalty is more exact modelling of the label noise -- 

\paragraph{Theoretical justification based on linear models.}
So far, the introduction of our approach is a bit high-level. To rigorously justify our method, we theoretically investigate our method based upon a simplified overparameterized linear model with sparse corruptions. As justified by a line of recent work \cite{jacot2018neural,chizat2018lazy}, overparameterized linear models capture similar phenoemona because they well approximate overparameterized deep networks in a linearized regime around the the initial points. Under sparse corruption and certain low-rank assumptions on the data, we show that the gradient descent \eqref{eq:main_algorithm} with an $\alpha$ below a certain threshold recovers the underlying model parameters with reasonably amounts of corruptions. Our result is obtained by explicitly characterizing the implicit regularization for the term $\u_i \odot \u_i - \v_i \odot \v_i$. In particular, we explicitly show that it leads to an $\ell_1$-norm regularization on the sparse corruption, hence connecting our method to classical $\ell_1$ loss approaches for model robustness. For more details, we refer readers to \Cref{sec:theory}. 

\qq{the following can be removed if not enough space}
\paragraph{Highlights of our contribution.} In summary, our contributions are two-folds:
\begin{itemize}[leftmargin=*]
    \item \emph{Method.} We proposed a simple yet practical SOP method that can effectively prevent overfitting for learning overparameterized deep networks from corrupted training data, demonstrated on a variety of datasets.
    \item \emph{Theory.} Under a simplified overparameterized linear model, we rigorously justifies our approach for exactly separating sparse corruption from the data.
\end{itemize}
Moreover, we believe the methodology we developed here could be far beyond the label noise setting, with potentials for dealing more challenging scenarios of robustly learning overparametrized models without overfitting.

%The result not only provides correctness guarantee for our method but also offers guideline for choosing $\alpha$, the only hyper-parameter introduced in our method. 

%See Section~\ref{sec:theory} for details.  The result not only provides correctness guarantee for our method but also offers guideline for choosing $\alpha$, the only hyper-parameter introduced in our method. 


%We provide a theoretical study of our method by applying it to an over-parameterized \emph{linear} model.A linear model is a commonly used special case for studying over-parameterized models \cite{hastie2019surprises} which well-approximates deep neural networks in a linearized regime around the initial point \cite{jacot2018neural,chizat2018lazy}. Under certain low-rank assumptions on the linear model, we show that
% Intuitively, it may appear that the negative effect of label noise can never be fully removed as it incurs a loss of information. 
% Our analysis shows, perhaps very surprisingly, that \emph{exact} recovery of the underlying clean label and model can be achieved under the linear model. 
% Informally, we show
%\begin{quote}
%    \em Algorithm in \eqref{eq:main_algorithm} with an $\alpha$ below a certain threshold recovers the underlying model parameters if the percentage of corrupted label is low.
%\end{quote}

% A particular benefit of linear models is that the implicit regularization of the gradient descent algorithm can be explicitly characterized by the $\ell_2$ norm. 


%it is important to note that our approach counters the classical wisdom that using more learnable parameters aggravates, rather than alleviates, the overfitting issue.
%By reading the formulation \eqref{eq:main_model} it indeed looks problematic: one of its global solutions is $\u_i \equiv \0, \v_i \equiv \0$ and $f(\x_i, \mb \theta) \equiv \y_i$ for all $i$ which is an overfitting solution.
%In fact, there are infinitely many global solutions to \eqref{eq:main_model} and overwhelmingly many of them do not address the overfitting problem at all. 
% Such a perspective, however, neglects the fact that a particular algorithm for solving \eqref{eq:main_model} determines which global solution the model converges to -- a phenomenon that is dubbed \emph{algorithmic bias} or \emph{implicit bias} [].
%Hence, an indispensable component of our approach is a particular algorithm for optimizing \eqref{eq:main_model}, which with proper design provides an implicit regularization with desired properties. % converges to a particular global solution with desired properties of $\u_i$ and $\v_i$ that are explained above. 
%In particular, our method requires solving \eqref{eq:main_model} via a gradient descent algorithm with different learning rates for $\mb \theta$ and $\{\u_i, \v_i\}$.
%Denoting the objective function in \eqref{eq:main_model} as $L(\mb \theta, \{\u_i, \v_i\})$, our algorithm starts with a small initial value of $\{\u_i, \v_i\}$ and updates the parameters with
%\begin{equation}\label{eq:main_algorithm}
%\begin{split}
%    \mb \theta &\leftarrow \mb \theta - \eta \cdot \frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \mb \theta},\\
%    \u_i &\leftarrow \u_i - \alpha \eta \cdot \frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \u_i},~~i=1, \ldots, N,\\
%    \v_i &\leftarrow \v_i - \alpha \eta \cdot\frac{\partial L(\mb \theta, \{\u_i, \v_i\})}{\partial \v_i},~~i=1, \ldots, N,\\
%\end{split}
%\end{equation}
%where $\alpha > 0$ is a tuning parameter. 



